Meta-Prompting for Automating Zero-shot Visual Recognition with LLMs

Prompt ensembling of Large Language Model (LLM) generated category-specific prompts has emerged as an effective method to enhance zero-shot recognition ability of Vision-Language Models (VLMs). To obtain these category-specific prompts, the present methods rely on hand-crafting the prompts to the LLMs for generating VLM prompts for the downstream tasks. However, this requires manually composing these task-specific prompts and still, they might not cover the diverse set of visual concepts and task-specific styles associated with the categories of interest. To effectively take humans out of the loop and completely automate the prompt generation process for zero-shot recognition, we propose Meta-Prompting for Visual Recognition (MPVR). Taking as input only minimal information about the target task, in the form of its short natural language description, and a list of associated class labels, MPVR automatically produces a diverse set of category-specific prompts resulting in a strong zero-shot classifier. MPVR generalizes effectively across various popular zero-shot image recognition benchmarks belonging to widely different domains when tested with multiple LLMs and VLMs. For example, MPVR obtains a zero-shot recognition improvement over CLIP by up to 19.8% and 18.2% (5.0% and 4.5% on average over 20 datasets) leveraging GPT and Mixtral LLMs, respectively

==> figs/abl_model_size_b_16.tex <==
\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{figs/accuracy_results_ViT-B_16.pdf}}
    \caption{Mean over 20 Datasets}
    \label{fig:Ablation:ViT_b16_results}
\end{figure*}

==> figs/abl_model_size_l_14.tex <==
\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{figs/accuracy_results_ViT-L_14.pdf}}
    \caption{Mean over 20 Datasets}
    \label{fig:Ablation:ViT_l14_results}
\end{figure*}

==> figs/abl_w_wo_cls.tex <==
\begin{figure}
    \centering
    \includegraphics{figs/bar_plot_w_wo_cls.pdf}
    \caption{Caption}
    \label{fig:abl:with_without_cls}
\end{figure}

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Vision-Language Models (VLMs)~\cite{clip,metaclip, instructblip, llava} have recently shown strong zero-shot recognition performance on various benchmarks. 
% Their ability to generalize to novel concepts in an open-vocabulary paradigm makes these large-scale foundation models extremely versatile. 
% The contrastively pre-trained dual encoder models (\eg CLIP~\cite{clip})
% These models are usually trained on a large corpus of paired text-image data, which allows them models to generalize to novel concepts in an open-vocabulary paradigm. 
Trained on a large corpus of paired text-image data allows these models to generalize to novel concepts in an open-vocabulary paradigm. 
% They utilize the shared image-text embedding space learned by the dual encoder models~\cite{clip, metaclip} during their large-scale pre-training, 
% and perform zero-shot recognition by searching for the maximum similarity between the query image embedding and the set of text embeddings of the class prompts. 
Leveraging the shared image-text embedding space learned by the dual encoder models~\cite{clip, metaclip}, the zero-shot recognition is performed by searching for the maximum similarity between the query image embedding and the set of text embeddings of the class prompts. 
For example, the most basic \emph{class prompts} could simply be \texttt{`a photo of a \{classname\}'} (the \emph{default} template), where \texttt{classname} is replaced by an arbitrary category for which recognition needs to be performed. 

It is empirically shown that obtaining the text embeddings using the \emph{default} template instead of only the \texttt{classname} results in better recognition performance. 
However, it is also noted in~\cite{clip} that the default template might be too generic for obtaining the text embeddings for task-specific images. 
For example, for the image of a flower, obtaining the text embedding by manipulating the input prompt to \texttt{`a photo of a \{classname\}, which is a flower'}, results in significantly better accuracy. 
Constructing a strong zero-shot classifier by the mean embeddings obtained by several of these dataset-specific hand-crafted templates (referred to as prompt ensembling in~\cite{clip}) results in impressive gains over using the default template but comes with the caveat that these ensembles have to be manually hand-crafted for each dataset.
\input{figs/motivation_2}

% \input{figs/motivation_2}
Following the idea of prompt ensembling in CLIP~\cite{clip}, CUPL~\cite{cupl} substituted the prompts with category-level descriptions
% proposed to obtain category-level descriptions 
by prompting an LLM with handcrafted prompts, manually crafted specifically for the dataset of interest for which recognition needs to be performed. 
Alternatively, DCLIP~\cite{dclip} proposed to replace category-level descriptions with category-level attributes obtained by asking an LLM to convert a category to a list of individually recognizable attributes. 
Similarly, Waffle-CLIP~\cite{waffle} also leverages LLM-generated category-level attributes and further adds random hand-crafted (per dataset) descriptors to broad concepts. 
These approaches take important steps towards automating category-level descriptions and enhancing the zero-shot recognition accuracy but: (i) still rely on hand-crafted prompts to the LLM (CUPL~\cite{cupl}) or manually designed dataset-specific broad concepts~(Waffle-CLIP~\cite{waffle}); and/or (ii) rely on individually recognizable attributes (DCLIP~\cite{dclip}) leading to somewhat limited zero-shot performance improvements (\eg for categories with diverse possible attribute combinations).
% In our work, we aim to reduce the manual effort spent on constructing the templates for ensembling or hand-crafting the dataset-specific prompts to be fed to the LLM for generating the category-level descriptions.

In this work, we aim to automate the prompt generation process, while further improving the zero-shot recognition performance of VLMs, beyond previous approaches.
% while further improving the accuracy of VLMs zero-shot recognition performance 
% beyond previous approaches.
As downstream categories of interest can potentially have countless visual variability, hand-crafting LLM prompts for describing them in natural language in all the possible diverse ways, visual styles, viewpoints, and contexts in which they may appear on images requires an exhaustive human effort, is not scalable, and may result in degraded performance. 
To counter this, we tap into the visual world knowledge learned by the LLMs during their large-scale autoregressive pre-training on an abundant text corpus without incurring additional manual effort for hand-crafting the prompts and propose \textbf{MPVR}: \textbf{M}eta \textbf{P}rompting for \textbf{V}isual \textbf{R}ecognition.

Our \method takes inspiration from~\cite{metaprompting, metaprompting1, icl} and proposes a general framework that essentially \textit{meta-prompts LLMs to produce prompt templates tailored to a downstream task via task description in a zero-shot manner}, consequently automating and improving the zero-shot visual recognition performance of VLMs. 
Given an in-context description of a dataset (downstream task description) and a fixed (downstream-task-independent) set of in-context prompt demonstrations, we generate target task category prompts in two consecutive calls to an LLM (\eg~Mixtral~\cite{mixtral}). 
%together with a system prompt (instruction) to generate a diverse set of prompts for another dataset for which we aim to perform zero-shot recognition. 
%
We first meta-prompt the LLM to generate a diverse and downstream-task adapted set of \emph{prompt templates}, each containing a \texttt{<category name>} placeholder. Second, for each downstream category, we populate its label into all the prompt templates generated in step one and prompt the LLM the second time, obtaining the desired diverse set of category-level prompts used as an ensemble for generating a robust zero-shot classifier for enhanced zero-shot visual recognition. An overview of \method is provided in Figure \ref{fig:motivation}. 
% After generating these diverse sets of prompts for our target dataset of interest, in order to extract diverse visual concepts for a category of interest, we again prompt the LLM with these prompts after populating them with the \texttt{<category name>} to obtain the category-level descriptions, as depicted in Figure~\ref{fig:motivation}. 
% These diverse descriptions are then used as an ensemble for generating a robust zero-shot classifier. 
Our Meta Prompting strategy is agnostic to the type of dataset for which we need to generate the prompts and only requires the knowledge of the dataset name and its description, which can easily be gathered through public APIs or obtained from its webpage. 
MPVR covers diverse visual concepts and visual styles related to the type of downstream dataset of interest resulting in impressive gains on a variety of zero-shot benchmarks with the added advantage of eliminating humans from the loop.
Our contributions can be summarized as follows: 

\begin{itemize}
    \item We propose a general framework for tapping into the visual world knowledge possessed by the LLMs through Meta Prompting which relies on gradient-free in-context learning and is completely automated, only requiring a generic description of the downstream task of interest.  
    \item Our proposed \method generalizes beyond closed models (like GPT~\cite{gpt3}) and for the first time we show that category-specific descriptions generated from open-source models (like Mixtral~\cite{mixtral}) can also enhance the zero-shot recognition abilities of state-of-the-art VLMs when evaluated on a diverse set of $20$ in-domain, out-of-domain and fine-grained classification datasets.  
    \item We open-source a dataset of $\sim2.5\text{M}$ unique category-level text descriptions harnessed from GPT and Mixtral with our meta-prompting framework, comprising the first massive-scale comprehensive textual dataset encompassing the breadth of LLM knowledge of the visual world.
    % which can lead to many exciting future work directions 
    % like instruction-tuning of VLMs to gain a better understanding of categories present in our world.    
\end{itemize}






==> sections/method.tex <==
\section{MPVR: Meta Prompting for Visual Recognition}
\label{sec:method}

% Dual-encoder VLMs~\cite{clip, metaclip} consist of a vision encoder and a text encoder which are usually pre-trained with a self-supervised contrastive objective on a large corpus of paired image-text data scraped from the web (\eg 400m).
% The underlying objective is to pull the embeddings of the same image-text pairs closer while pushing away the embeddings from unrelated image-text pairs. 
% CLIP~\cite{clip} shows that the shared image-text embedding space learned by these VLMs enables them to be strong zero-shot (open-vocabulary) classifiers.
% For classification,
% given the set of class names $\ClassNames$, the text encoder $\txtEnc$ is used to generate the embedding $t_c = \txt(c)$ of a prompt for each class $\cls\in\ClassNames$,
% typically of the form `\texttt{A photo of \{classname\}}', which is complemented with the class name.
% Similarly, each test image $\img$ is encoded by the vision encoder $\visEnc$, and the classification is performed 
% % on its cosine similarity $\simil$ to the text embedding of the prompt, populated with the name of each class.
% according to max cosine similarity $\simil$ to the best matching category prompt embedding.
% %
% % Finally, t
% The likelihood of a predicted class $\hat\cls$ is computed with a softmax,
% \begin{equation} \label{eq:zeroshot}
% \likel_{\hat\cls}(\img) = \frac{e^{\simil(\txtEmbNew,\visEnc(\img))/{\tau}}}{\sum_{\cls\in\ClassNames} e^{\simil(\txtEmb,\visEnc(\img))/{\tau}}} ,
% \end{equation}
% where $\tau$ denotes the temperature constant.

The zero-shot classifier in Eq.~\eqref{eq:zeroshot} can perform classification in an open vocabulary paradigm and requires no additional training data. 
In CLIP~\cite{clip} it is shown that instead of using the default prompt `\texttt{A photo of a <class name>}', the zero-shot classification can be further enhanced by obtaining the text embeddings through an ensemble of hand-crafted dataset-specific prompts\footnoteref{footnote:prompt-ensemble-clip}. 
%\footnotemark[\value{footnote}].
% ~\ref{footnote:prompt-ensemble-clip}.
Given a set of dataset-specific prompts $P = \{p_1, p_2, \ldots, p_n\}$, the text embedding for a class $\cls$ for zero-shot classification is the mean of the embeddings from $P$ after inserting the \texttt{<class name>} at the placeholders,

\begin{equation}
    \txtEmb_c = \frac{1}{n} \sum_{i=1}^{n} \txtEnc(p_i).
    \label{eq:mean_text_emb}
\end{equation}



% Following this idea,~\cite{cupl, dclip, waffle} proposed to obtain 
% the text embeddings by ensembling 
% by leveraging large language models to generate category-level descriptions (or attributes) for the categories in a dataset.  

Following this idea, \cite{cupl, dclip, waffle, tap} proposed to obtain the \emph{prompts} in the form of category-level descriptions (or attributes) by leveraging a large language model (\eg GPT~\cite{gpt3}). 
Although these approaches can enhance the performance of the zero-shot classifiers, often they require manual construction of the prompts to the LLM for each type of data expected in the downstream set of images which is not scalable. 
Furthermore, even if it was possible to manually construct prompts for each type of data expected to be encountered, it might require an exhaustive human effort to creatively design prompts that cover the diverse ways the visual aspects of a certain category can be described in the text.  

In contrast, we propose a two-step approach MPVR, aimed at relieving humans from the burden of composing these task-specific prompts.
In the first step, given a set of example demonstrations and coarse information about the downstream task of interest, \method generates multiple diverse task-specific prompts (for the LLMs) through meta-prompting.
These task-specific prompts enable our \method to tap into the visual world knowledge possessed by the VLMs about the categories of interest tailored towards the visual style of the task.
In the second stage, these task-specific prompts are populated with the \texttt{<class name>} of interest and fed again to the LLM to obtain fine-grained category-specific prompts used for constructing a zero-shot classifier through ensembling.
% by tasking an LLM to first generate a diverse set of prompts with Meta Prompting for any type of data.
% these are prompts to an LLM that allow leveraging its visual world knowledge about categories of interest
% b. these prompts are task-specific, they are already infused with the information of visual styles of the task
% c. after populating them with categories we can get information about the particular category (from the LLM worl knowledge) in the visual style of the task
% and then later using these prompts to generate the category-specific descriptions.   
An overview of our methodology is provided in Figure~\ref{fig:main}.
In Section~\ref{subsec:method:meta-prompting} we describe how to effectively \emph{prompt LLMs for diverse prompts} and later in Section~\ref{subsec:method:category-level-descriptions} we describe the second stage of generating category-level descriptions from these diverse set of prompts. 
In addition to reducing the manual effort, our two-step approach also helps us to achieve a state-of-the-art zero-shot classifier when tested on diverse benchmarks and VLMs while comparing to relevant baselines. 
We provide these results in Section~\ref{sec:results}.
\input{figs/main_fig}


\subsection{Meta Prompting}
\label{subsec:method:meta-prompting}
% Present-day large language models have been trained on an enormous corpus of text data that is scraped from the web (\eg GPT~\cite{gpt3}). 
% The extensive pre-training of these language models allows them to learn a \textit{world model}, enabling them to impressively describe a variety of concepts in our world. 
The extensive pre-training of large language models on an enormous corpus of web-scraped text data (\eg GPT~\cite{gpt3}) allows them to learn a \textit{world model}, enabling them to impressively describe a variety of concepts in our world.
Moreover, the variability in the training data also allows these strong models to describe visual concepts present in our world. 
To extract the knowledge condensed in the weights of these large models, a significant amount of effort has been spent on proposing different techniques for effectively prompting these networks~\cite{icl, cot, expertprompting, treeofthought, kojima2022large} for obtaining impressive gains on multiple natural language tasks. 

Inspired by the vibrant literature on prompting for natural language processing~\cite{icl,cot, treeofthought}, here we present a novel prompting method for extracting the visual world knowledge from LLMs to guide the contrastively pre-trained VLMs for enhanced zero-shot classification. 
At a higher level, the underlying goal of our proposed Meta Prompting is to prompt the LLMs to generate multiple diverse prompts.
% The template used by our Meta Prompting framework is provided in Figure~\ref{fig:motivation}.
Our Meta Prompting provides a generic framework and can be used to generate diverse sets of prompts for any kind of task-specific data but for simplicity of explanation, here we consider the example of a dataset used for benchmarking purposes. 
As illustrated in Figure~\ref{fig:meta-prompting}, the Meta Prompt employed by our \method is composed of three main parts. 
First, a System Prompt provides a comprehensive instruction set that describes the different parts of the entire Meta Prompt and provides exact instructions about what is expected as output from the LLM (\eg~prompts formatted in a \texttt{Python} script).
Second, the in-context example of a dataset, and third the dataset metadata for a downstream dataset of interest. 
% Specifically explaining what is provided in the Meta Prompt (\eg~the example dataset)  and what is expected 
More specifically, we assume that we have access to an in-context example of a dataset for which we are provided the dataset name, metadata (dataset description), and the corresponding prompts for this dataset which are hand-crafted.
Aligned with our goal of generating a diverse set of prompts for any dataset of interest for which we want to tap into the visual world knowledge of the LLM -- given the name of this dataset, we first scrape the metadata for this dataset from a public API (\eg~GitHub).
This metadata only contains a generic description of the type of data expected to be encountered in a particular dataset. 
\input{figs/motivation}
For example, to generate the prompts for the type of data present in the ImageNet-Rendition dataset~\cite{imagenet-r}, the following metadata is scraped from Github: 
\quotebox{{ImageNet-R(endition) contains art, cartoons, deviantart, graffiti, embroidery, graphics, origami, paintings, patterns, plastic objects, plush objects, sculptures, sketches, tattoos, toys, and video game renditions of ImageNet classes.}}
Next, we populate the metadata, along with the in-context dataset example in the template we outline in Figure~\ref{fig:motivation}.
This Meta Prompt is then fed to the LLM (\eg~GPT~\cite{gpt3} or Mixtral~\cite{mixtral})
to generate $N$ diverse prompts for the downstream dataset of interest.

Our Meta Prompting framework alleviates the need for human involvement in the creative process of composing the dataset-specific prompts and instead provides the reigns to the LLM to generate these prompts.
This is in contrast to the previous methods that rely on hand-crafting of the prompts~\cite{cupl, tap, waffle} for obtaining the category-level descriptions, and since their prompt generation strategy requires manual effort, they are not able to utilize the vast knowledge base of the LLMs for visually describing the categories of interest in the downstream dataset. 

% To this end, next, we describe how we use these prompts to arrive at our final goal of obtaining category-level descriptions for the composition of a strong zero-shot classifier. 

% We insert this in-context example into the Meta Prompting template shown in Figure~\ref{fig:motivation} and the Meta Prompt is then fed to the LLM to generate 



% to generate category-level descriptions by feeding the prompts to an LLM.
% For a specific dataset of interest, given the name of this dataset, we first scrape the metadata for this dataset from a public API (\eg~GitHub, Hugging Face~\etc). 
% Then we complement the 

% . with the corresponding prompts used to generate multiple descriptions for it,

\subsection{Category-Level Descriptions}
\label{subsec:method:category-level-descriptions}
The Meta Prompt instructs the LLM to generate a variety of prompts for a downstream dataset and conveniently formats them to be employed in a \texttt{Python} script for use in the second stage of our \method (following our instructions in the System Prompt).
The prompts generated as a response to our Meta Prompt are generic, but contain a placeholder for the \texttt{class name} of interest. 
To formulate these prompts in a manner that helps us to obtain category-level descriptions, we replace the \texttt{class name} with the actual category of interest, and 
% Finally, after populating these generic prompts with the \texttt{class name}, we 
feed them to the LLM, resulting in various category-level descriptions. 
% Since, these category-level descriptions are generated from a huge variety of prompts, these 
Generating these descriptions from various prompts helps us to extract the visual world knowledge possessed by the LLMs more effectively. 
For zero-shot classification, given a test image $\img$, the softmax classification probabilities are obtained by utilizing Eq.~\eqref{eq:zeroshot}. However, instead of obtaining the text embeddings from the default prompt provided by CLIP~\cite{clip} or the ensemble of prompts, we construct the zero-shot classifier from the mean of the text embeddings from our category-level text descriptions obtained from Eq.~\eqref{eq:mean_text_emb}.


We repeat this procedure for each category in our downstream dataset with both the GPT~\cite{gpt3} and Mixtral~\cite{mixtral} LLMs for $20$ different datasets (used for evaluating our \method) and obtain a huge corpus of $\sim2.5\text{M}$ diverse category-level descriptions, which is already incorporated in our codebase provided in the supplementary material and will be open-sourced upon acceptance. 





==> sections/method_prev_intro.tex <==
\section{MPVR: Meta Prompting for Visual Recognition}
\label{sec:method}

Dual-encoder VLMs~\cite{clip, metaclip} consist of a vision encoder and a text encoder which are usually pre-trained with a self-supervised contrastive objective on a large corpus of paired image-text data scraped from the web (\eg 400m).
The underlying objective is to pull the embeddings of the same image-text pairs closer while pushing away the embeddings from unrelated image-text pairs. 
CLIP~\cite{clip} shows that the shared image-text embedding space learned by these VLMs enables them to be strong zero-shot (open-vocabulary) classifiers.
For classification,
given the set of class names $\ClassNames$, the text encoder $\txtEnc$ is used to generate the embedding $t_c = \txt(c)$ of a prompt for each class $\cls\in\ClassNames$,
typically of the form `\texttt{A photo of \{classname\}}', which is complemented with the class name.
Similarly, each test image $\img$ is encoded by the vision encoder $\visEnc$, and the classification is performed 
% on its cosine similarity $\simil$ to the text embedding of the prompt, populated with the name of each class.
according to max cosine similarity $\simil$ to the best matching category prompt embedding.
%
% Finally, t
The likelihood of a predicted class $\hat\cls$ is computed with a softmax,
\begin{equation} \label{eq:zeroshot}
\likel_{\hat\cls}(\img) = \frac{e^{\simil(\txtEmbNew,\visEnc(\img))/{\tau}}}{\sum_{\cls\in\ClassNames} e^{\simil(\txtEmb,\visEnc(\img))/{\tau}}} ,
\end{equation}
where $\tau$ denotes the temperature constant.

The zero-shot classifier in Eq.~\eqref{eq:zeroshot} can perform classification in an open vocabulary paradigm and requires no additional training data. 
In CLIP~\cite{clip} it is shown that instead of using the default prompt `\texttt{A photo of a \{classname\}}', the zero-shot classification can be further enhanced by obtaining the text embeddings through an ensemble of hand-crafted dataset-specific prompts\footnoteref{footnote:prompt-ensemble-clip}. 
%\footnotemark[\value{footnote}].
% ~\ref{footnote:prompt-ensemble-clip}.
Given a set of dataset-specific prompts $P = \{p_1, p_2, \ldots, p_n\}$, the text embedding for a class $\cls$ for zero-shot classification is the mean of the embeddings from $P$ after inserting the class name at the placeholders,

\begin{equation}
    \txtEmb = \frac{1}{n} \sum_{i=1}^{n} \theta_t(p_i).
    \label{eq:mean_text_emb}
\end{equation}



% Following this idea,~\cite{cupl, dclip, waffle} proposed to obtain 
% the text embeddings by ensembling 
% by leveraging large language models to generate category-level descriptions (or attributes) for the categories in a dataset.  

Following this idea, \cite{cupl, dclip, waffle, tap} proposed to obtain the \emph{prompts} in the form of category-level descriptions (or attributes) by leveraging a large language model (\eg GPT~\cite{gpt3}). 
Although these approaches can enhance the performance of the zero-shot classifiers, often they require manual construction of the prompts to the LLM for each type of data expected in the downstream set of images which is not scalable. 
Furthermore, even if it was possible to manually construct prompts for each type of data expected to be encountered, it might require an exhaustive human effort to creatively design prompts that cover the diverse ways the visual aspects of a certain category can be described in the text.  
In contrast, we propose a two-step approach MPVR aimed at relieving humans from the burden of composing these task-specific prompts by tasking an LLM to first generate a diverse set of prompts with Meta Prompting for any type of data and then later using these prompts to generate the category-level descriptions.   
An overview of our methodology is provided in Figure~\ref{fig:main}.
In Section~\ref{subsec:method:meta-prompting} we describe how to effectively \emph{prompt LLMs for diverse prompts} and later in Section~\ref{subsec:method:category-level-descriptions} we describe the second stage of generating category-level descriptions from these diverse set of prompts. 
In addition to reducing the manual effort, our two-step approach also helps us to achieve a state-of-the-art zero-shot classifier when tested on diverse benchmarks and VLMs while comparing to relevant baselines. 
We provide these results in Section~\ref{sec:results}.
\input{figs/main_fig}


\subsection{Meta Prompting}
\label{subsec:method:meta-prompting}
% Present-day large language models have been trained on an enormous corpus of text data that is scraped from the web (\eg GPT~\cite{gpt3}). 
% The extensive pre-training of these language models allows them to learn a \textit{world model}, enabling them to impressively describe a variety of concepts in our world. 
The extensive pre-training of large language models on an enormous corpus of web-scraped text data (\eg GPT~\cite{gpt3}) allows them to learn a \textit{world model}, enabling them to impressively describe a variety of concepts in our world.
Moreover, the variability in the training data also allows these strong models to describe visual concepts present in our world. 
To extract the knowledge condensed in the weights of these large models, a significant amount of effort has been spent on proposing different techniques for effectively prompting these networks~\cite{icl, cot, expertprompting, treeofthought, kojima2022large} for obtaining impressive gains on multiple natural language tasks. 

Inspired by the vibrant literature on prompting for natural language processing~\cite{icl,cot, treeofthought}, here we present a novel prompting method for extracting the visual world knowledge from LLMs to guide the contrastively pre-trained VLMs for enhanced zero-shot classification. 
At a higher level, the underlying goal of our proposed Meta Prompting is to prompt the LLMs to generate multiple diverse prompts.
% The template used by our Meta Prompting framework is provided in Figure~\ref{fig:motivation}.
Our Meta Prompting provides a generic framework and can be used to generate diverse sets of prompts for any kind of task-specific data but for simplicity of explanation, here we consider the example of a dataset used for benchmarking purposes. 
As illustrated in Figure~\ref{fig:meta-prompting}, the Meta Prompt employed by our \method is composed of three main parts. 
First, a System Prompt provides a comprehensive instruction set that describes the different parts of the entire Meta Prompt and provides exact instructions about what is expected as output from the LLM (\eg~prompts formatted in a \texttt{Python} script).
Second, the in-context example of a dataset, and third the dataset metadata for a downstream dataset of interest. 
% Specifically explaining what is provided in the Meta Prompt (\eg~the example dataset)  and what is expected 
More specifically, we assume that we have access to an in-context example of a dataset for which we are provided the dataset name, metadata (dataset description), and the corresponding prompts for this dataset which are hand-crafted.
Aligned with our goal of generating a diverse set of prompts for any dataset of interest for which we want to tap into the visual world knowledge of the LLM -- given the name of this dataset, we first scrape the metadata for this dataset from a public API (\eg~GitHub).
This metadata only contains a generic description of the type of data expected to be encountered in a particular dataset. 
\input{figs/motivation}
For example, to generate the prompts for the type of data present in the ImageNet-Rendition dataset~\cite{imagenet-r}, the following metadata is scraped from Github: 
\quotebox{{ImageNet-R(endition) contains art, cartoons, deviantart, graffiti, embroidery, graphics, origami, paintings, patterns, plastic objects, plush objects, sculptures, sketches, tattoos, toys, and video game renditions of ImageNet classes.}}
Next, we populate the metadata, along with the in-context dataset example in the template we outline in Figure~\ref{fig:motivation}.
This Meta Prompt is then fed to the LLM (\eg~GPT~\cite{gpt3} or Mixtral~\cite{mixtral})
to generate $N$ diverse prompts for the downstream dataset of interest.

Our Meta Prompting framework alleviates the need for human involvement in the creative process of composing the dataset-specific prompts and instead provides the reigns to the LLM to generate these prompts.
This is in contrast to the previous methods that rely on hand-crafting of the prompts~\cite{cupl, tap, waffle} for obtaining the category-level descriptions, and since their prompt generation strategy requires manual effort, they are not able to utilize the vast knowledge base of the LLMs for visually describing the categories of interest in the downstream dataset. 

% To this end, next, we describe how we use these prompts to arrive at our final goal of obtaining category-level descriptions for the composition of a strong zero-shot classifier. 

% We insert this in-context example into the Meta Prompting template shown in Figure~\ref{fig:motivation} and the Meta Prompt is then fed to the LLM to generate 



% to generate category-level descriptions by feeding the prompts to an LLM.
% For a specific dataset of interest, given the name of this dataset, we first scrape the metadata for this dataset from a public API (\eg~GitHub, Hugging Face~\etc). 
% Then we complement the 

% . with the corresponding prompts used to generate multiple descriptions for it,

\subsection{Category-Level Descriptions}
\label{subsec:method:category-level-descriptions}
The Meta Prompt instructs the LLM to generate a variety of prompts for a downstream dataset and conveniently formats them to be employed in a \texttt{Python} script for use in the second stage of our \method (following our instructions in the System Prompt).
The prompts generated as a response to our Meta Prompt are generic, but contain a placeholder for the \texttt{class name} of interest. 
To formulate these prompts in a manner that helps us to obtain category-level descriptions, we replace the \texttt{class name} with the actual category of interest, and 
% Finally, after populating these generic prompts with the \texttt{class name}, we 
feed them to the LLM, resulting in various category-level descriptions. 
% Since, these category-level descriptions are generated from a huge variety of prompts, these 
Generating these descriptions from various prompts helps us to extract the visual world knowledge possessed by the LLMs more effectively. 
For zero-shot classification, given a test image $\img$, the softmax classification probabilities are obtained by utilizing Eq.~\eqref{eq:zeroshot}. However, instead of obtaining the text embeddings from the default prompt provided by CLIP~\cite{clip} or the ensemble of prompts, we construct the zero-shot classifier from the mean of the text embeddings from our category-level text descriptions obtained from Eq.~\eqref{eq:mean_text_emb}.


We repeat this procedure for each category in our downstream dataset with both the GPT~\cite{gpt3} and Mixtral~\cite{mixtral} LLMs for $20$ different datasets (used for evaluating our \method) and obtain a huge corpus of $\sim2.5\text{M}$ diverse category-level descriptions, which is already incorporated in our codebase provided in the supplementary material and will be open-sourced upon acceptance. 





==> supp_sections/erratum.tex <==
\section{Erratum}
\label{sec:supp:erratum}

In the main manuscript Table $4$, the \method accuracy for CIFAR-100~\cite{cifar} should actually be $66.3\%$ (consistent with the results reported in Table $1$ of the main manuscript for the same ViT-B/32 backbone from CLIP~\cite{clip}), which is higher than the $64.4\%$ that we reported in Table $4$ by mistake. %Sorry!


==> supp_sections/truncating_prompts.tex <==
\section{Truncating VLM prompts}
\label{sec:supp:truncating_VLM_prompts}

\input{tables/descriptiveness_of_descriptions}

To explore the effect of \emph{descriptiveness} of our LLM-generated VLM prompts, we design an experiment where we truncate the prompts for each class with a fixed window size, randomly chosen between $50\%\to70\%$ for each description (VLM prompt) but we take care that the class name is not removed if it was included in the original description. 
These results are provided in Table~\ref{tab:trunate-descriptions}, where we report the average of $5$ random runs when truncating the descriptions. 
These results indicate that the CLIP text encoder responds well to syntactically correct (and descriptive) sentences, further highlighting the reason why our \method performs better than Waffle~\cite{waffle}, which adds random descriptors to high-level concepts.


==> supp_tables/incontext_dataset_ablation.tex <==
\begin{table}[t!]
    \centering
                    \setlength{\tabcolsep}{10pt}

    \begin{tabular}{llc}
    \toprule
         in-context dataset & target dataset &top-1 (\%)\\
         \midrule
         \midrule
        Flowers & DTD&52.0\\
                EuroSAT & DTD &50.8\\

        CUBS & DTD&51.8\\
         \midrule


         Flowers & EuroSAT&54.5\\
         CUBS &EuroSAT&54.4\\
                          DTD & EuroSAT&55.6\\

         \bottomrule
         \bottomrule
    \end{tabular}
    \caption{Top-1 accuracy (\%) with ViT-B/32~\cite{clip} while using different datasets as the in-context example dataset in the stage-1 of \method (meta-prompting).}
    \label{tab:in_context_dataset_ablation}
\end{table}

==> tables/descriptiveness_of_descriptions.tex <==
% \begin{table*}[]
%     \centering
%     % \resizebox{0.7\textwidth}{!}{
%         \setlength{\tabcolsep}{10pt}

%     \begin{tabular}{c|cccc}
%     \toprule
%          &  GPT & Mixtral & GPT - CLS & Mixtral - CLS\\
%         \midrule
%         \midrule
%        ViT-B32 & {62.9} & {62.4} & {44.9} & {24.0} \\
% ViT-B16 & {66.7} & {66.4} & {48.5} & {25.5} \\
% ViT-L14 & {73.4} & {72.5} & {55.2} & {28.4} \\
%         \bottomrule
%         \bottomrule
%     \end{tabular}
%     % }
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}
\begin{table}[t!]
\small
        \setlength{\tabcolsep}{8pt}

    \centering
    \begin{tabular}{l|cc|cc}
\toprule

 & GPT & Mixtral & Truncated GPT & Truncated Mixtral \\
\midrule
\midrule

ViT-B/32 & {62.9} & {62.4} & {56.2} & {55.5} \\
ViT-B/16 & {66.7} & {66.4} & {59.8} & {60.2} \\
ViT-L/14 & {73.4} & {72.5} & {67.6} & {67.1} \\
\bottomrule
\bottomrule

\end{tabular}
    \caption{Comparison of mean top-1 accuracy (\%) over 20 datasets obtained by using the complete description set for \method (first two columns) and truncating the text descriptions with a fixed window.}
    \label{tab:trunate-descriptions}
\end{table}
% \begin{tabular}{lrrr}
% \toprule
%  & GPT & Mixtral & Truncated GPT \\
% \midrule
% ViT-B_32 & {62.9} & {62.4} & {56.2} \\
% ViT-B_16 & {66.7} & {66.4} & {59.8} \\
% ViT-L_14 & {73.4} & {72.5} & {67.6} \\
% \bottomrule
% \end{tabular}


==> tables/results_stability.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{c|cc}
    \toprule
                    & accuracy(\%)& std\\
                    \midrule
                    \midrule
         ViT-B/32& 62.8 & $\pm$0.05\\
         ViT-B/16& 66.7 & $\pm$0.04\\
         ViT-L/14& 73.3 & $\pm$0.03\\
         \bottomrule
         \bottomrule
    \end{tabular}
    \caption{Top-1 mean accuracy (\%) and standard deviation for $10$ random runs.}
    \label{tab:my_label}
\end{table}

==> tables/softmax_ensembling.tex <==
\begin{table*}[]
\small
    \centering
        \setlength{\tabcolsep}{2pt}

    \resizebox{1\textwidth}{!}{
    \begin{tabular}{c|cccccc}
    \toprule
         &  GPT & Mixtral & GPT+Temp & Mixtral+Temp & GPT+Mixtral& GPT+Mixtral+Temp\\
        \midrule
        \midrule
ViT-B/32 & \textbf{62.9} & {62.4} & \underline{62.8} & {62.3} & {62.4} & {62.4} \\
ViT-B/16 & \textbf{{66.7}} & \underline{66.4} & \textbf{{66.7}} & \underline{66.4} & \underline{66.4} & {66.3} \\
ViT-L/14 & \textbf{{73.4}} & {72.5} & \underline{73.3} & {72.4} & {72.6} & {72.6} \\
        \bottomrule
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of mean top-1 accuracy (\%) for MPVR over 20 datasets while constructing
the zero-shot classifier by averaging the individual softmax probabilities.}
    \label{tab:ensembling-text-with-softmax-average}
\end{table*}
